Multi-Frame to Single-Frame: Knowledge Distillation for 3D Object Detection

A common dilemma in 3D object detection for autonomous driving is that high-quality, dense point clouds are only available during training, but not testing. We use knowledge distillation to bridge the gap between a model trained on high-quality inputs at training time and another tested on low-quality inputs at inference time. In particular, we design a two-stage training pipeline for point cloud object detection. First, we train an object detection model on dense point clouds, which are generated from multiple frames using extra information only available at training time. Then, we train the model's identical counterpart on sparse single-frame point clouds with consistency regularization on features from both models. We show that this procedure improves performance on low-quality data during testing, without additional overhead.

==> section/ablation.tex <==
\section{Ablation Study}
This is ablation.

==> section/acknowledgement.tex <==
\section{Acknowledgements}
This is ack

==> section/conclusion.tex <==
\section{Conclusion}
We present a two-stage training pipeline for point cloud object detection, tackling the data mismatch problem between training and testing. Our key observation in this paper is that a model can make use of the privileged information at training time via a simple knowledge distillation procedure. In addition, this framework preserves inference efficiency at test time. 

Our pipeline can be incorporated as-is into any object detection model for point clouds. Beyond its direct usage, our experiments suggest several future directions. One immediate extension is to investigate whether other knowledge distillation variants can further improve the model; for example, we can leverage recently proposed contrastive learning-based objectives, such as CRD~\cite{tian2019contrastive}. Furthermore, the large amount of unlabeled data available at training time can serve as another 
type of privileged information. This data suggests the promise of applying \emph{self-supervised learning} to 3D domains, which remains a largely open problem.
%\jw{The last sentence is a little too speculative to me.}

%is also aligned with self-supervised learning, which has set to be worthily applied to 3D domain.

%is still much under study in 3D domain.

% In addition, 3D reconstruction 

% \yue{also talk about full observation at training, partial observation at testing, e.g, 3D reconstruction}

==> section/impact.tex <==
\section*{Broader Impacts}
The goal of this paper is to improve the object detection pipeline, which is crucial for the safety of autonomous driving systems. We hope this work can contribute to bringing self driving cars (or autonomous systems more broadly) to reality sooner, to reduce traffic accidents, and to increase productivity. Future work to improve applicability in this domain might consider challenges of \emph{explainability}, which currently elude popular object detection models.

==> section/related_work.tex <==
\section{Related Work}
% \paragraph{Learning on point clouds.} \justin{this paragraph seems unnecessary to me, and also looks suspiciously similar to analogous paragraphs in our past work.  consider removing it (why bother citing a billion point cloud networks?) and make sure the wording is different than past work.}Deep sets~\cite{Zaheer2017} and PointNet~\cite{Qi_2017_CVPR} pioneered deep learning on point sets, a challenging problem in learning and vision. These methods usually include two parts: a shared multi-layer perceptrons (MLPs) to take coordinates with additional point-wise features as input, and embed them into high-dimensional space; a symmetric function to aggregate features over the point set. However, these methods only consider the global structure and ignore local geometry of shapes. To address that, PointNet++~\cite{qi2017pointnetplusplus} applies PointNet in each local sphere to learn local geometric features. DGCNN~\cite{dgcnn} further generalizes learning local features using graph neural networks~\cite{kipf2016semi,Monti17} and introduces a non-local operation similar to self-attention in image processing~\cite{NonLocal2018}\justin{broken reference} and natural language processing~\cite{Vaswani2017}. PCNN~\cite{pcnn2018} maps point cloud functions to volumetric functions and vice versa, using extension and restriction operators. SPLATNet~\cite{Su2018SPLATNetSL} projects point clouds to lattice grid and performs lattice convolutions. To introduce extra flexibility of the convolutional kernels, KPConv~\cite{thomas2019kpconv} defines deformable convolutions using a set of kernel points. For fast processing, PCVNN~\cite{liu2019pvcnn} learns fine-grained point features to compensate coarse voxel representations. Rather than rendering point clouds to dense grids, MinkowskiNet~\cite{choy20194d} and Sparse ConvNet~\cite{sparseconv} introduce sparse convolutional operations tailored to processing sparse data. Beyond working on high-level recognition tasks, recent works~\cite{Wang2019DCP,Wang2019PRNetSL,Goforth2019,Sarode2019OneFT,choy2019fully,choy2020deep} tackle the low-level registration problems with point cloud networks; they showcase these low-level tasks can also benefit from learning priors directly from data. Furthermore, FlowNet3D~\cite{flownet3d} and MeteorNet~\cite{Liu_2019_ICCV} study dynamical point clouds and show learning flow estimation is effective with point cloud networks.  

\paragraph{3D object detection.} 3D object detection is a major application of learning on point clouds. VoxelNet~\cite{Zhou_2018_CVPR} generalizes one-stage object detection models to 3D; in particular, it uses 3D dense convolutions to learn representations on the voxelized point clouds, which is not efficient enough to capture fine-grained features. To address that, PIXOR~\cite{Yang2018PIXORR3} and PointPillars~\cite{Lang_2019_CVPR} both project points to a birds-eye view (BEV) and operate on 2D feature maps. A PointNet~\cite{qi2017pointnet} is used to aggregate features within each BEV pixel. These methods, although more efficient, largely drop information along the vertical axis. To accompany the birds-eye view projection, MVF~\cite{Zhou2019EndtoEndMF} proposes using additional spherical projection to learn complementary information. In addition to these SSD-style~\cite{liu2016ssd} object detection models, Complex-YOLO~\cite{Simon2018ComplexYOLOR3} extends YOLO to 3D and achieves real-time 3D perception. PointRCNN~\cite{shi2019pointrcnn} employs a two-stage architecture to perform high-quality detection. 

In contrast to works on point clouds, LaserNet~\cite{Meyer2019LaserNetAE} instead operates on raw range scans and achieves comparable performance. To incorporate additional information, recent works~\cite{ku2018joint,Chen2016Multiview3O,Xu2017PointFusionDS} combine point clouds with camera images to utilize complementary representations from both modalities. Frustum-PointNet~\cite{qi2017frustum} leverages 2D object detectors to form a frustum crop of points and then uses a PointNet to aggregate features from points in the frustum. \cite{Liang_2018_ECCV} designed an end-to-end learnable architecture that exploits continuous convolutions to fuse feature maps at every level. 
VoteNet~\cite{qi2019deep, qi2020imvotenet} generalizes Hough voting~\cite{Hough} for 3D object detection in point clouds. DOPS~\cite{Najibi2020DOPSLT} extends VoteNet and predicts 3D shapes of the objects at the same time. 
In addition to visual inputs, \cite{yang18b} shows that High-Definition (HD) maps can help boost the performance of 3D object detectors. \cite{Liang_2019_CVPR} argues that multi-tasking training can help the network to learn better representations than single-tasking. Beyond supervised learning, \cite{Wong2019IdentifyingUI} investigates how to learn a perception model for unknown classes. In our pipeline, we use a variant of PointPillars~\cite{Lang_2019_CVPR} for 3D detection. 

\paragraph{Knowledge distillation.} The original goal of knowledge distillation (KD)~\cite{Bucilua2006} is to compress the knowledge contained in an ensemble of models into a single smaller model. \cite{knowledgedistillation} generalizes this idea and combines it with deep learning. Knowledge distillation transfers the knowledge from a teacher model to a student model by minimizing a loss, in which the target is the distribution of class probabilities induced by the teacher model.
%It was shown in \cite{yim2017} that KD has several benefits for optimization and knowledge transfer between tasks. 
In addition to the original approach in which a small network imitates the %soft 
output of a larger network, many follow-up works improve various aspects of the pipeline. FitNets~\cite{Romero15-iclr} proposes matching intermediate representations of the student network to those of the teacher network. Attention Transfer~\cite{Zagoruyko2017AT} focuses on the feature maps of the network as opposed to the final outputs, eliciting similar response patterns in the teacher and student feature maps. SPKD~\cite{Tung2019SimilarityPreservingKD} improves Attention Transfer by preserving pairwise similarities of feature maps. Relational KD~\cite{Park2019RelationalKD} learns to transfer mutual relations of data examples. FSP~\cite{Yim_2017_CVPR} views the distilled knowledge to be dense flow transferred between layers. CRD~\cite{tian2019crd} connects knowledge distillation to representation learning via a contrastive objective~\cite{Oord2018RepresentationLW,he2019moco,chen2020simple,tian2019contrastive}. Self-distillation is a special case of knowledge distillation, where the teacher model and student model have the same capacity. BAN~\cite{FurlanelloLTIA18} introduces sequential self-distillation, which distills knowledge from the model's latest snapshot. In natural language processing (NLP), BAM~\cite{clark2019bam} uses BAN to distill from single-task models to a multi-task model, enabling the multi-task model to surpass its single-task teachers. 

Beyond image classification, knowledge distillation has been extended to improve object detection. \cite{NIPS2017_6676} leverages FitNets for object detection and addresses obstacles such as class imbalance, loss instability, and feature distribution mismatch. \cite{LiJY17} performs distillation only between region proposals, which amplifies fast training but leads to instability. To address this issue, \cite{Wang_2019_CVPR} proposes fine-grained representation imitation using object masks. 
% Moreover,\justin{$\leftarrow$ weird transition}
\cite{Liu2020ContinualUO} uses knowledge distillation to tackle a continual learning problem in object detection. Our model makes use of privileged information during training to transfer knowledge between 3D point cloud--based object detection models. 

\paragraph{Learning using privileged information.} \cite{VapnikV09} introduces the framework of learning with privileged information in the context of support vector machines (SVMs), which deals with the case when additional information is accessible during training but not testing. \cite{LopSchBotVap16} unifies knowledge distillation and learning using privileged information from the theoretical perspective. %\justin{by doing what?}. 
\cite{su2017adapting} identifies practical scenarios where this idea can be applied, e.g., transferring knowledge from localized data to non-localized data, from high resolution to low resolution, from color images to edge images, and from regular images to distorted images. To control the uncertainty of the model output and improve training efficiency, \cite{Lambert_2018_CVPR} makes the variance of Dropout~\cite{srivastava14a} a function of privileged information. Our work is a natural extension of these methods to 3D data, in which the privileged information consists of dense point clouds aggregated from sequences of LiDAR scans. 

% \yue{say about the connection between ours and LURI.}
